Adaptive Phase-Shifted Pilot Design for Uplink Multiple Access in ISAC Systems

In uplink integrated sensing and communication (ISAC) systems, pilot signal design is crucial for enabling accurate channel estimation and reliable radar sensing. In orthogonal frequency-division multiple access (OFDMA)-based frameworks, conventional pilot allocation schemes face a trade-off between spectral efficiency (SE) and sensing performance. Interleaved pilots improve user equipment (UE) multiplexing through sparse allocation but reduce the maximum unambiguous range. Conversely, orthogonal block-based pilots reduce range ambiguity but degrade sensing resolution due to limited delay granularity. To address this trade-off, the phase-shifted ISAC (PS-ISAC) scheme was recently proposed for uplink multiple access in ISAC systems. However, PS-ISAC suffers from spectral inefficiency due to the fixed cyclic prefix (CP) constraints. To overcome these limitations, we propose adaptive phase-shifted-ISAC (APS-ISAC), an enhanced pilot scheme that employs an overlapped block-pilot structure with UE-specific phase shifts determined by maximum excess delay of each UE. This design enables UEs to share the same time-frequency resources while preserving separable and contiguous channel impulse responses (CIRs) at the base station (BS). Simulation results show that APS-ISAC significantly outperforms conventional pilot allocation methods in terms of SE, approximately doubling the number of multiplexed UEs. It also achieves lower mean square error (MSE) under power constraints with reduced complexity. Furthermore, it yields maximum range resolution and unambiguous sensing performance. These results establish APS-ISAC as a scalable, spectrally efficient, ambiguity-resilient, and low-complexity pilot design paradigm for future uplink ISAC systems.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{UE}[UE]{user equipment}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{ISAC}[ISAC]{integrated sensing and communications}
\acrodef{IFFT}[IFFT]{inverse fast Fourier transform}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{FFT}[FFT]{FFT}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{LS}[LS]{least-square}
\acrodef{MMSE}[MMSE]{minimum mean-square error}
\acrodef{BPSK}[BPSK]{binary phase shift keying}
\acrodef{CI-ISAC}[CI-ISAC]{conventional interleaved-ISAC}
\acrodef{CB-ISAC}[CB-ISAC]{conventional block-ISAC}
\acrodef{PS-ISAC}[PS-ISAC]{phase-shifted-ISAC}
\acrodef{APS-ISAC}[APS-ISAC]{adaptive phase-shifted-ISAC}
\acrodef{MSE}[MSE]{mean-square error}
\acrodef{NOMA}[NOMA]{non-orthogonal multiple access}
\acrodef{OOBE}[OOBE]{out-of-band emissions}
\acrodef{OFDMA}[OFDMA]{orthogonal frequency-division multiple access}
\acrodef{CFR}[CFR]{channel frequency response}
\acrodef{FPR}[FPR]{full pilot ratio}
\acrodef{PR}[PR]{pilot ratio}
\acrodef{MUR}[MUR]{maximum unambiguous range}
\acrodef{MA}[MA]{multiple access}
\acrodef{NGMA}[NGMA]{next-generation MA}
\acrodef{PRS}[PRS]{positioning RS}
\acrodef{UL}[UL]{uplink}
\acrodef{DL}[DL]{downlink}
\acrodef{CC}[CC]{computational complexity}
\acrodef{PC}[PC]{power constraints}
\acrodef{DMRS}[DMRS]{demodulation RS}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{SE}[SE]{spectral efficiency}
\acrodef{MED}[MED]{maximum excess delay}
\acrodef{LSE}[LSE]{least-square estimation}
\acrodef{TRX}[TRX]{transceiver}
\acrodef{TX}[TX]{transmitter}
\acrodef{RX}[RX]{receiver}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{XR}[XR]{extended reality}
\acrodef{IoT}[IoT]{internet of things}
\acrodef{TF}[TF]{time-frequency}
\acrodef{CRB}[CRB]{Cramér–Rao bound}
\acrodef{MAC}[MAC]{multiple access channel}
\acrodef{CPI}[CPI]{coherent processing interval}
\acrodef{ISI}[ISI]{inter symbol interference}
\acrodef{PS}[P/S]{parallel-to-serial}
\acrodef{SP}[S/P]{serial-to-parallel}
\acrodef{DAC}[DAC]{digital-to-analog conversion}
\acrodef{ADC}[ADC]{analog-to-digital conversion}
\acrodef{AIC}[AIC]{Akaike information criterion}
\acrodef{MDL}[MDL]{minimum description length}
\acrodef{RCS}[RCS]{radar cross section}
\acrodef{ICI}[ICI]{inter carrier interference}
\acrodef{PLS}[PLS]{physical layer security}
\acrodef{PDF}[PDF]{probability density function}
\acrodef{TTI}[TTI]{transmission time interval}
\acrodef{CFAR}[CFAR]{constant false alarm rate}
\acrodef{LTE}[LTE]{long-term evolution}
\acrodef{5G}[5G]{5th generation}
\acrodef{6G}[6G]{6th generation}
\acrodef{NR}[NR]{new radio}
\acrodef{RF}[RF]{reciprocal filtering}
\acrodef{ZF}[ZF]{zero-forcing}
\acrodef{UE}[UE]{user equipment}
\acrodef{BS}[BS]{base station}
\acrodef{IID}[IID]{independent and identically-distributed}
\acrodef{RS}[RS]{reference signal}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
